Time-series machine-learning error models for approximate solutions to parameterized dynamical systems

This work proposes a machine-learning framework for modeling the error incurred by approximate solutions to parameterized dynamical systems. In particular, we extend the machine-learning error models (MLEM) framework proposed in Ref. 15 to dynamical systems. The proposed Time-Series Machine-Learning Error Modeling (T-MLEM) method constructs a regression model that maps features--which comprise error indicators that are derived from standard a posteriori error-quantification techniques--to a random variable for the approximate-solution error at each time instance. The proposed framework considers a wide range of candidate features, regression methods, and additive noise models. We consider primarily recursive regression techniques developed for time-series modeling, including both classical time-series models (e.g., autoregressive models) and recurrent neural networks (RNNs), but also analyze standard non-recursive regression techniques (e.g., feed-forward neural networks) for comparative purposes. Numerical experiments conducted on multiple benchmark problems illustrate that the long short-term memory (LSTM) neural network, which is a type of RNN, outperforms other methods and yields substantial improvements in error predictions over traditional approaches.

==> error_analysis.tex <==
We first derive \textit{a posteriori} error bounds for \textit{any} arbitrary
sequence of approximate solutions $\stateApprox^\tindx(\parametervec)$,
$\tindx=0,\ldots,\ntimesteps$. This analysis borrows strongly from the error
bounds derived in Ref.~\cite{leeCarlberg}.

\begin{theorem}[Normed state error: \textit{a posteriori} bound]\label{thm:error_bound}
	If the velocity $\velo$ is Lipschitz continuous, i.e.,
	there exists a constant $\lipschitz>0$ such that
	$\norm{\velo(\bm{x},t;\parametervec)-\velo(\bm{y},t;\parametervec)}\leq\lipschitz\norm{\bm{x}-\bm{y}}$
	for all $\bm{x},\,\bm{y}\in\RR{\nstate}$ and
	$t\in\{t^\tindx\}_{i=1}^{\ntimesteps}$, and
	the time step is sufficiently small such that
	$ \Delta t < {\abs{\alpha_0}}/{\abs{\beta_0}\lipschitz}$,
	then 
\begin{equation} \label{eq:finalGenResult}
	\norm{\stateFOMArg{n}\paramDep - \stateROMArg{n}\paramDep}\leq\frac{1}{\hconstant}
	\norm{\resnROMParamsArg{\stateROMArg{n}\paramDep}} +
\sum_{j=1}^{\kArg{n}}\gammaconstantj\norm{
\stateFOMArg{n-j}(\parametervec)-\stateROMArg{n-j}(\parametervec)
		}
\end{equation} 
for all $n=1,\ldots,\ntimesteps$.
	Here, $\hconstant\defeq\abs{\alpha_0} - \abs{\beta_0}\lipschitz\Delta t$
and $\gammaconstantj\defeq\left(\abs{\alpha_j} + 
	\abs{\beta_j}\lipschitz
	\Delta
	t\right)/\hconstant$.
\end{theorem}
\begin{proof}
	For notational simplicity, we suppress dependence on the parameters
	$\parametervec$ in the proof.
Subtracting  $\resnROMArg{\stateROMArg{n}}$ from $\resnFOMArg{\stateFOMArg{n}}$ and
noting from 
Eq.~\eqref{eq:fom_discretized} that $\resnFOMArg{\stateFOMArg{n}} =
\zero$ yields
\begin{align*} 
\begin{split} 
	-\resnROMArg{\stateROMArg{n}} =& \alpha_0\left(\stateFOMArg{n} -
	\stateROMArg{n}\right) - \Delta
	t\beta_0\left(\velo(\stateFOMArg{n},t^n)-\velo(\stateROMArg{n},t^n)\right)\\
	 &+ \sum_{j=1}^{\kArg{n}} \alpha_j
	 \left(\stateFOMArg{n-j}-\stateROMArg{n-j}\right)
	- \Delta t \sum_{j=1}^{\kArg{n}} \beta_j \left(\velo
	(\stateFOMArg{n-j},t^{n-j})
	-\velo (\stateROMArg{n-j},t^{n-j})\right).
\end{split} 
\end{align*} 
Rearranging this expression gives
\begin{align} \label{eq:IandII}
\begin{split} 
	&\underbrace{\stateFOMArg{n} - \stateROMArg{n} - 
	\frac{\Delta
	t\beta_0}{\alpha_0}\left(\velo(\stateFOMArg{n},t^{n})-\velo(\stateROMArg{n},t^{n})\right)}_\text{(I)}
	 =\\
	&\qquad\underbrace{-\frac{1}{\alpha_0}\resnROMArg{\stateROMArg{n}} -  \frac{1}{\alpha_0}\sum_{j=1}^{\kArg{n}} \alpha_j
	 \left(\stateFOMArg{n-j}-\stateROMArg{n-j}\right)
	+ \frac{\Delta t}{\alpha_0} \sum_{j=1}^{\kArg{n}} \beta_j \left(\velo
	(\stateFOMArg{n-j},t^{n-j})
	-\velo (\stateROMArg{n-j},t^{n-j})\right)}_\text{(II)}.
\end{split} 
\end{align} 
We proceed by bounding $\norm{\text{(I)}}$ from below, and $\norm{\text{(II)}}$ from above.
To bound $\norm{\text{(I)}}$ from below, we apply the reverse triangle to obtain
 \begin{equation} \label{eq:Iboundone}
	 \norm{\text{(I)}}\geq
	 \abs{
	 \norm{\stateFOMArg{n} - \stateROMArg{n}} - 
	 \norm{\underbrace{
\frac{\Delta
	 t\beta_0}{\alpha_0}\left(\velo(\stateFOMArg{n},t^{n})-\velo(\stateROMArg{n},t^{n})\right)
		 }_\text{(I.a)}}
	 }.
 \end{equation}
 We now use Lipschitz continuity of the velocity $\velo$ to bound
 $\norm{\text{(I.a)}}$ from above as
\begin{equation} \label{eq:Iboundtwo}
\norm{
	\text{(I.a)}
}\leq \frac{\Delta t
		 \abs{\beta_0}\lipschitz}{\abs{\alpha_0}}\norm{\stateFOMArg{n} -
		 \stateROMArg{n}}.
\end{equation} 
If time-step-restriction condition $ \Delta t < {\abs{\alpha_0}}/{\abs{\beta_0}\lipschitz}$ holds,
then we can combine inequalities \eqref{eq:Iboundone} and \eqref{eq:Iboundtwo}
as
\begin{equation} \label{eq:Ilowerbound}
\norm{\text{(I)}}\geq
	 \frac{\hconstant}{\abs{\alpha_0}}\norm{\stateFOMArg{n} - \stateROMArg{n}}.
\end{equation} 

To bound $\norm{\text{(II)}}$ in Eq.~\eqref{eq:IandII} from above, we apply the triangle
inequality and employ Lipschitz continuity of the velocity $\velo$, which
gives
\begin{equation} \label{eq:IIupperbound}
	\norm{
		\text{(II)}
		}\leq
	\frac{1}{\abs{\alpha_0}}\norm{\resnROMArg{\stateROMArg{n}}}
	+ \frac{1}{\abs{\alpha_0}}\sum_{j=1}^{\kArg{n}}\left(\abs{\alpha_j} + 
	\abs{\beta_j}\lipschitz
	\Delta
	t\right)\norm{
\stateFOMArg{n-j}-\stateROMArg{n-j}
		}.
\end{equation} 
Combining Eq.~\eqref{eq:IandII} with inequalities \eqref{eq:Ilowerbound} and
\eqref{eq:IIupperbound} gives the desired result.
\end{proof}


==> error_analysis_qoi.tex <==
\begin{corollary}[Normed QoI error: \textit{a posteriori} bound]
Under the assumptions of Theorem \ref{thm:error_bound} and additionally
assuming Lipschitz continuity of the QoI functional $\qoiFunc$, i.e.,
	i.e.,
	there exists a constant $\lipschitzQoI>0$ such that
	$\abs{\qoiFuncArgs{\bm{x}}{t}{\parametervec}-\qoiFuncArgs{\bm{y}}{t}{\parametervec}}\leq\lipschitzQoI\norm{\bm{x}-\bm{y}}$
	for all $\bm{x},\,\bm{y}\in\RR{\nstate}$ and
	$t\in\{t^\tindx\}_{i=1}^{\ntimesteps}$, and
	the time step is sufficiently small such that
	$ \Delta t < {\abs{\alpha_0}}/{\abs{\beta_0}\lipschitz}$,
	then 
\begin{equation} \label{eq:finalGenResultQoI}
	\abs{\qoiArg{n}\paramDep -
	\qoiApproxArg{n}\paramDep}\leq\frac{\lipschitzQoI}{\hconstant}
	\norm{\resnROMParamsArg{\stateROMArg{n}\paramDep}} +
\lipschitzQoI\sum_{j=1}^{\kArg{n}}\gammaconstantj\norm{
\stateFOMArg{n-j}(\parametervec)-\stateROMArg{n-j}(\parametervec)
		}
\end{equation} 
for all $n=1,\ldots,\ntimesteps$.
	Constants $\hconstant$
and $\gammaconstantj$ are defined in Theorem \ref{thm:error_bound}.
\end{corollary}
\begin{proof}
The proof follows trivially from Lipschitz continuity and the bound in 
Theorem \ref{thm:error_bound}.
\end{proof}


==> error_bounds.tex <==

\subsubsection{A Posteriori Error Bounds for the Solution Norm}
\textit{A posteriori} error bounds for the Galerkin reduced-order model are now derived. It is assumed that the velocity of the dynamical system is Lipschitz continuous: there exists some $\kappa > 0$ such that, $\forall \mathbf{v},\mathbf{w} \in \mathbb{R}^N$,
$$\norm{ \velocityFOM (\mathbf{v},\parametervec)  - \velocityFOM(\mathbf{w}  ,\parametervec) } \le \kappa \norm{ \mathbf{v} - \mathbf{w} }.$$
A projection-based reduced-order model obeys the following dynamical system,
\begin{equation}\label{eq:gromerror}
\projectionROM \bigg[\frac{d \statevecROM}{dt}-  \velocityFOM(\statevecROM,\parametervec) \bigg]= \mathbf{0}, \qquad \statevecROM(0) = \statevec_0,
\end{equation}
Subtracting Eq.~\ref{eq:gromerror} from Eq.~\ref{eq:fom} yields,
\begin{equation}\label{eq:gromerror}
 \bigg[ \fomeq \bigg] - \projectionROM \bigg[\frac{d \statevecROM}{dt}-  \velocityFOM(\statevecROM,\parametervec) \bigg]   = \mathbf{0}, \qquad \statevecROM(0) = \statevec_0,
\end{equation}

\begin{equation}\label{eq:gromerror}
 \bigg[ \fomeq \bigg] - \bigg[\projectionROM - \mathbf{I} + \mathbf{I} \bigg] \bigg[\frac{d \statevecROM}{dt}-  \velocityFOM(\statevecROM,\parametervec) \bigg]   = \mathbf{0}, \qquad \statevecROM(0) = \statevec_0,
\end{equation}

\begin{equation}\label{eq:gromerror}
 \bigg[ \frac{d \error}{dt} - \velocityFOM( \statevec,\parametervec) + \velocityFOM(\statevecROM,\parametervec) \bigg] +  \bigg[ \mathbf{I} - \projectionROM \bigg] \bigg[\frac{d \statevecROM}{dt}-  \velocityFOM(\statevecROM,\parametervec) \bigg]   = \mathbf{0}, \qquad \statevecROM(0) = \statevec_0,
\end{equation}

\begin{equation}\label{eq:gromerror}
\frac{d \error}{dt} = \bigg[ \velocityFOM( \statevec,\parametervec) - \velocityFOM(\statevecROM,\parametervec) \bigg] - \bigg[ \mathbf{I} - \projectionROM \bigg] \bigg[\frac{d \statevecROM}{dt}-  \velocityFOM(\statevecROM,\parametervec) \bigg] , 
\end{equation}

\begin{equation}\label{eq:gromerror}
\frac{d \norm{ \error } }{dt} \le \kappa \norm{ \error} + \norm{ \bigg[\mathbf{I}-  \projectionROM \bigg] \bigg[ \velocityFOM(\statevecROM,\parametervec) - \frac{d \statevecROM}{dt}  \bigg]},
\end{equation}

\begin{equation}\label{eq:rom_error_f}
\norm{ \error(t) } = \int_0^t e^{ \kappa s } \norm{ \bigg[\mathbf{I}-  \projectionROM \bigg] \bigg[ \velocityFOM(\statevecROM(t-s),\parametervec) - \frac{d \statevecROM}{dt}(t-s)  \bigg]} ds 
\end{equation}
Equation ~\ref{eq:rom_error_f} demonstrates that the error is non-local in time, i.e. the state error at the current time instance is dependent on the history of the solution residual. Although Eq.~\ref{eq:rig_bound} is rigorous, it is not necessarily useful as it indicates exponential growth in the error with a growth rate that scales by the (positive) Lipshitz constant $\kappa$. 

\begin{comment}
\subsubsection{Approximate Linearized Error Bounds}
An alternative to computing rigorous error bounds is to compute approximate error bounds. This work considers approximate error bounds obtained through linearization. By making the linearized assumption,
$$ \mathbf{R}(\mathbf{u},\mu) \approx \mathbf{R}(\statevecROM,\mu) + \frac{\partial \mathbf{R}}{\partial \mathbf{u}} \delta(\mu,t),$$ 
the following error bounds can be derived,
\begin{equation}\label{eq:error_bounds_linearized}
||\delta(t)|| \le \int_0^t || \mathbf{S} e^{\Lambda s} \mathbf{S}^{-1} \mathbf{r}(\statevecROM(t-s),\mu) || ds. 
\end{equation}
{\color{red} This is for LTI. Need to finish for non-linear.}
\end{comment}
\subsection{Dual Weighted Residual Error Bounds}
Typically, QoI error is quantified through dual weighted residuals. Two formulations of the dual weighted residual are formualted here: the local dual-weighted residual and the full dual-weighted residual.

\subsubsection{Time Continuous Adjoint}
Definition of the adjoint
$$\MC{J}(\delta \statevec) = \int_0^t \adjointvec^T \mathbf{r}'( \delta \statevec) d t,$$
where 
$$\mathbf{r}(\statevec) = \frac{d \statevec}{dt} - \velocityFOM(\statevec)$$
First pertubation is,
$$\mathbf{r}'(\delta \statevec) = \frac{d}{dt}\delta \statevec - \frac{\partial \velocityFOM}{\partial \mathbf{v}}[\statevec] \delta \statevec.$$
Thus,
$$\MC{J}(\delta \statevec) = \int_0^t \adjointvec^T \bigg( \frac{d \delta \statevec}{dt} - \frac{\partial \velocityFOM}{\partial \mathbf{v}}[\statevec] \delta \statevec \bigg)  d t.$$
Integrating by parts and transposing,
$$\MC{J}^T(\delta \statevec) = \int_0^t \delta \statevec^T \bigg( -\frac{d \adjointvec}{dt} - \frac{\partial \velocityFOM}{\partial \mathbf{v}}[\statevec]^T \adjointvec \bigg)  d t.$$
As,
$$\MC{J}(\delta \statevec) = \int_0^t \frac{\partial g}{\partial \mathbf{v}}[\statevec] \delta \statevec dt,$$
We have,
$$\int_0^t  \delta \statevec^T \frac{\partial g}{\partial \mathbf{v}}^T[\statevec] dt  = \int_0^t \delta \statevec^T \bigg( -\frac{d \adjointvec}{dt} - \frac{\partial \velocityFOM}{\partial \mathbf{v}}[\statevec]^T \adjointvec \bigg)  d t.$$
Define the adjoint to be the solution of,
$$ \frac{d \adjointvec}{dt} + \frac{\partial \velocityFOM}{\partial \mathbf{v} }[\statevec]^T \adjointvec= -\frac{\partial g}{\partial \statevec}^T[\statevec], \qquad \adjointvec(T) = 0.$$
QoI definition:
$$\MC{J}(\statevec) = \int_0^t g \big( \statevec(t) , t \big)dt.$$
Then
$$\MC{J}(\statevec) - \MC{J}(\statevecROM)  = \int_0^t g \big(\statevec(t),t \big)) - g\big(\statevecROM(t),t \big)  dt.$$
$$\MC{J}(\statevec) - \MC{J}(\statevecROM)  \approx \int_0^t \frac{\partial g}{\partial \mathbf{v}}[\statevecROM] \big(\statevec(t) - \statevecROM(t)) dt.$$
$$\MC{J}(\statevec) - \MC{J}(\statevecROM)  \approx \int_0^t \bigg( \frac{d \adjointvec}{dt} + \frac{\partial \velocityFOM}{\partial \mathbf{v} }[\statevec]^T \adjointvec \bigg) \big(\statevec(t) - \statevecROM(t)) dt.$$
$$\MC{J}(\statevec) - \MC{J}(\statevecROM)  \approx \int_0^t \adjointvec^T \bigg( \frac{d \statevec}{dt} - \frac{\partial \velocityFOM}{\partial \mathbf{v} }[\statevec] \statevec  -  \frac{d \statevecROM}{dt} + \frac{\partial \velocityFOM}{\partial \mathbf{v} }[\statevec] \statevecROM \bigg) dt.$$
$$\MC{J}(\statevec) - \MC{J}(\statevecROM)  \approx -\int_0^t \adjointvec^T \bigg( \frac{d \statevecROM}{dt} - \frac{\partial \velocityFOM}{\partial \mathbf{v} }[\statevecROM] \statevecROM \bigg) dt.$$
$$\MC{J}(\statevec) - \MC{J}(\statevecROM)  \approx -\int_0^t \adjointvec^T \mathbf{r}'(\statevecROM) dt.$$
\begin{comment}
\subsubsection{Time Local Dual Weighted Residual} 
At the $n_{th}$ entry, the one has,
$$\mathbf{r}(\statevec^n) = \mathbf{0}.$$
Writing as,
$$\mathbf{r}(\statevec^n) = \mathbf{r}(\statevecROM^N + \error^N) = \mathbf{0}.$$
Linearizing
$$ \mathbf{r}(\statevecROM^N + \error^N) = \mathbf{r}(\statevecROM^N) + \mathbf{J}[\statevecROM^N] \error^N + \mathcal{O}(\error^2).$$
The local error is then given by,
$$ \error^N = - \mathbf{J}[\statevecROM^N]^{-1} \mathbf{r}(\statevecROM^N).$$
Now consider the same QoI quantity,
$$\mathbf{g}(\statevec^N) = \mathbf{g}(\statevecROM^N + \error^N) = \mathbf{g}(\statevecROM^N) + \frac{\partial \mathbf{g}}{\partial \mathbf{v}} [\statevecROM^N] \error^N + \mathcal{O}(\error^2).$$ 
So,
$$\error^N = \frac{\partial \mathbf{g}}{\partial \mathbf{v}} [\statevecROM^N]^{-1} \Delta \mathbf{g}.$$
Subsituting in,
$$ \frac{\partial \mathbf{g}}{\partial \mathbf{v}}^{-1} [\statevecROM^N] \Delta \mathbf{g}= - \mathbf{J}[\statevecROM^N]^{-1} \mathbf{r}(\statevecROM^N).$$
Left multiplying by the inverse,
$$ \Delta \mathbf{g}= -\frac{\partial \mathbf{g}}{\partial \mathbf{v}} [\statevecROM^N]\mathbf{J}[\statevecROM^N]^{-1} \mathbf{r}(\statevecROM^N).$$
Typically, the term $\frac{\partial \mathbf{g}}{\partial \mathbf{v}} [\statevecROM^N]\mathbf{J}[\statevecROM^N]^{-1}$ is referred to as the dual or adjoint and is the solution to the dual problem,
$$ \mathbf{J}[\statevecROM^N]^T \mathbf{y}^N =  \frac{\partial \mathbf{g}}{\partial \mathbf{v}} [\statevecROM^N]^T.$$
Thus the QoI error can be approximated as,
$$\Delta g = {\mathbf{y}^N}^T \mathbf{r}(\statevecROM^N).$$
\end{comment}



==> noise_model.tex <==
At time instances
$n\in\timeIndexSet$,
we assume that we can compute $\nfeatures$ \textit{features}
$\featurenmu\in\mathbb{R}^{\nfeatures}$ that are informative of the error
of interest $\errorGennmu$. Section \ref{sec:featureEngineering} provides
candidate features, which are inspired by the classical error-quantification
methods described in Section \ref{sec:classicalError}.
Motivated by the approach pursued in Ref.~\cite{freno_carlberg_ml}, we 
propose constructing
\textit{a posteriori} error models of the form
\begin{equation}\label{eq:error_split}
\errorGennmu  \approx  \errorApproxMeanGennmu + \errorApproxRandGennmu,
\end{equation}
where $\errorApproxMeanGennmu: \parameterdomain \rightarrow \RR{}$ is a deterministic approximation to the error and $\errorApproxRandGennmu$ a mean-zero stochastic process. The deterministic approximation to the error is given by,
\begin{equation}\label{eq:ml_deterministic}
\errorApproxMeanGennmu =  \approxregressionfunction(\featurenmu,\latentstatefnmu),
\end{equation}
where $\approxregressionfunction: \RR{\nfeatures}\times\RR{\nlatentf}\rightarrow
\RR{}$ denotes the deterministic \textit{regression function} and
$\latentstatefn:\parameterdomain\rightarrow \RR{\nlatentf}$ is a set of \textit{latent
variables}. Critically, the inclusion of
latent variables enable the proposed method to capture non-local
temporal effects. In particular,
the latent variables are governed by the recursive relationships,
\begin{align}
	\latentstatefnmuArg{\timeIndexMapping{n}} &=
	\recursionf(\latentstatefnmuArg{\timeIndexMapping{n-1}},
	\errorApproxMeanGennmunArg{\timeIndexMapping{n-1}},
	\featurefnmuArg{\timeIndexMapping{n}}),\quad
	n=1,\ldots,\ntimestepsCoarse,
\end{align}
where $\recursionf:  \RR{\nlatentf}\times\RR{}\times\RR{\nfeatures}
\rightarrow
\mathbb{R}^{\nlatentf}$ 
defines the recursion for the deterministic regression function.

We make similar definitions for the stochastic process. Let,
\begin{equation}\label{eq:ml_stochastic}
\errorApproxRandGennmu =  \approxnoisefunction(\featureepsilonnmu,\latentstateepsilonnmu,\noiseArgs),
\end{equation}
where $\approxnoisefunction: \RR{\nfeaturesepsilon}\times\RR{\nlatentepsilon}\times\RR{}\rightarrow
\RR{}$ denotes the \textit{noise model},
$\latentstateepsilonn:\parameterdomain\rightarrow \RR{\nlatentepsilon}$ an additional vector of latent
variables, and $\epsilon: \RR{\nfeaturesepsilon}\times\RR{\nlatentepsilon} \rightarrow\RR{}$ a mean-zero random variable. The latent variables are governed by,  
\begin{equation}
        \latentstateepsilonnmuArg{\timeIndexMapping{n}} =
        \recursionepsilon(\latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}}, \vecnoise( \latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}} ) ), \qquad
%( \latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}} ),\quad
        n=1,\ldots,\ntimestepsCoarse,
\end{equation}
where $\recursionepsilon:   \RR{\nlatentepsilon}\times\RR{\nfeaturesepsilon} \times\RR{\nlatentepsilon} \rightarrow \RR{\nlatentepsilon}$ defines the regression function for the stochastic noise model, and $\vecnoise:  \RR{\nlatentepsilon}\times\RR{\nfeaturesepsilon} \rightarrow \RR{\nlatentepsilon} $ is a vector of mean-zero random variables. 

\begin{comment}
\textit{a posteriori} error models $\errorApproxGennmu(\approx\errorGennmu)$ of the form
\begin{equation}\label{eq:ml_framework}
\errorApproxGennmu =
	\approxregressionfunction(\featurenmu,\latentstatefnmu) +
	\approxnoisefunction(\featureepsilonnmu,\latentstateepsilonnmu) , \quad \tindx
	\in\timeIndexSet,
\end{equation}
where
$\approxregressionfunction: \RR{\nfeatures}\times\RR{\nlatentf}\rightarrow
\RR{}$ denotes the deterministic \textit{regression function},
$\approxnoisefunction:  \RR{\nfeaturesepsilon} \times \RR{\nlatentepsilon} \rightarrow \mathbb{R}$ is a stochastic noise model, and
$\latentstate^{\tindx}_f:\parameterdomain\rightarrow \mathbb{R}^{N_{h_f}}$ and
$\latentstate^{\tindx}_{\noise} :\parameterdomain\rightarrow \
\mathbb{R}^{N_{h_{\noise}}}$, $n\in\timeIndexSet$ denote
\textit{latent
variables}. Critically, the inclusion of
latent variables enable the proposed method to capture non-local
temporal effects.
%; this is in contrast to the approach pursued in
%Ref.~\cite{trehan_ml_error}, which attempts to model non-local effects by
%explicitly including quantities computed at previous time instances in the
%set of features. 
In particular,
the latent variables are governed by the recursive relationships,
\begin{align}
	\latentstatefnmuArg{\timeIndexMapping{n}} &=
	\recursionf(\latentstatefnmuArg{\timeIndexMapping{n-1}},
	\errorApproxGennmuArg{\timeIndexMapping{n-1}},
	\featurefnmuArg{\timeIndexMapping{n}}),\quad
	n=1,\ldots,\ntimestepsCoarse,\\
        \latentstateepsilonnmuArg{\timeIndexMapping{n}} &=
        \recursionepsilon(\latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}}) + \vecepsilon( \latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}} ),\quad
        n=1,\ldots,\ntimestepsCoarse,
%	\latentstateepsilonnmuArg{\timeIndexMapping{n}} &=
%	\recursionepsilon(\latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}}),\quad
%	n=1,\ldots,\ntimestepsCoarse,
\end{align}
where $\recursionf:  \RR{\nlatentf}\times\RR{}\times\RR{\nfeatures}
\rightarrow
\mathbb{R}^{\nlatentf}$ 
defines the recursion for the deterministic regression function, $\recursionepsilon:   \RR{\nlatentepsilon}\times\RR{\nfeaturesepsilon} \rightarrow \RR{\nlatentepsilon}$ defines the regression function for the stochastic noise model, and $\vecepsilon$ is a vector of mean-zero random variables. 

\end{comment}
%% Keep this to later put into the noise model section
\begin{comment}
\subsubsection{Gaussian/Laplacian Model}
For a Gaussian model set:
$$  \hat{X}(\featurenmu,\latentstateepsilonnmu)  = \latentstateepsilonnmu$$
$$\recursionepsilon(\latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}}) = 0$$
$$ \noise ( \latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}} ) \sim \MC{N}(0,\sigma(  \latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}}  ).$$
For laplacian change the distribution only. In the numerical experiments I use constant $\sigma$, so we could simplify.

\subsection{Autoregressive model}
For an autoregressive model of order $q$, take $\latentstateepsilonnmu \in \mathbb{R}^{q+1}$ and set,
$$  \hat{X}(\featurenmu,\latentstateepsilonnmu)  = \mathbf{w}^T \latentstateepsilonnmu,$$
$$ \recursionepsilon(\latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}}) = \begin{bmatrix}
\latentstateepsilonnmuArg{\timeIndexMapping{n-1}}_2\\
\latentstateepsilonnmuArg{\timeIndexMapping{n-1}}_3\\
\vdots \\
\latentstateepsilonnmuArg{\timeIndexMapping{n-1}}_{q+1}\\
\epsilon,
\end{bmatrix}
$$
where $\epsilon \sim \MC{N}(0,\sigma(  \latentstateepsilonnmuArg{\timeIndexMapping{n-1}},\featureepsilonnmuArg{\timeIndexMapping{n}}  ).$
\end{comment}

